Learning Variational Motion Prior for Video-based Motion Capture

Motion capture from a monocular video is fundamental and crucial for us humans to naturally experience and interact with each other in Virtual Reality (VR) and Augmented Reality (AR). However, existing methods still struggle with challenging cases involving self-occlusion and complex poses due to the lack of effective motion prior modeling. In this paper, we present a novel variational motion prior (VMP) learning approach for video-based motion capture to resolve the above issue. Instead of directly building the correspondence between the video and motion domain, We propose to learn a generic latent space for capturing the prior distribution of all natural motions, which serve as the basis for subsequent video-based motion capture tasks. To improve the generalization capacity of prior space, we propose a transformer-based variational autoencoder pretrained over marker-based 3D mocap data, with a novel style-mapping block to boost the generation quality. Afterward, a separate video encoder is attached to the pretrained motion generator for end-to-end fine-tuning over task-specific video datasets. Compared to existing motion prior models, our VMP model serves as a motion rectifier that can effectively reduce temporal jittering and failure modes in frame-wise pose estimation, leading to temporally stable and visually realistic motion capture results. Furthermore, our VMP-based framework models motion at sequence level and can directly generate motion clips in the forward pass, achieving real-time motion capture during inference. Extensive experiments over both public datasets and in-the-wild videos have demonstrated the efficacy and generalization capability of our framework.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/relatedwork_ref.tex <==
\begin{figure*}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/fig_2_overview}
	\caption{The pipeline of ChallenCap with multi-modal references. Assuming the video input from monocular camera, our approach consists of a hybrid motion inference stage (Sec.\ref{sec:mot_inference}) and a robust motion optimization stage (Sec.\ref{sec:mot_optimization}) to capture 3D challenging motions. $\mathcal{D}$ represents the discriminator. }  %\textcolor{red}{[Ma: Could we have descriptions or fill in content for the vacant boxes and trapezoid? In addition, give more description in the caption.]}
	\label{fig:overview}
\end{figure*}


\section{Related Work}
As an alternative to the widely used marker-based solutions~\cite{VICON,Xsens,Vlasic2007}, markerless motion capture~\cite{BreglM1998,AguiaSTAST2008,TheobASST2010} technologies alleviate the need for body-worn markers and have been widely investigated.
%
In the following, we focus on the field of marker-less 3D human motion capture.

\myparagraph{Parametric Model-based Capture.}
Many general human parametric models~\cite{SCAPE2005,SMPL2015,SMPLX2019,STAR_ECCV2020} learned from thousands of high-quality 3D scans have been proposed in the last decades, which factorize human deformation into pose and shape components. 
% human shape prior by using human parametric models 
Deep learning is widely used to obtain skeletal pose and human shape prior through model fitting~\cite{TAM_3DV2017,Lassner17,keepitSMPL,Kolotouros_2019_CVPR} or directly regressing the model parameters from the input~\cite{HMR18,Kanazawa_2019CVPR,VIBE_CVPR2020,zanfir2020neural}.
%
Besides, various approaches~\cite{detailHuman_2019CVPR,DetailDepth_2019ICCV,People3D_2019ICCV,TEX2SHAPE_2019ICCV,DeepHuman_2019ICCV} propose to predict detailed human geometry by utilizing parametric human model as a basic estimation.
%
Beyond human shape and pose, recent approaches further include facial and hand models~\cite{Xiang_2019_CVPR,TotalCapture,SMPLX2019,MonoExpressive_ECCV2020} for expressive reconstruction or leverage garment and clothes modeling on top of parametric human model~\cite{ClothCap,bhatnagar2019mgn,TailorNet_CVPR2020,LearnToDress_CVPR2020}.
%
But these methods are still limited to the parametric model and cannot provide space-time coherent results for loose clothes. 
%
Instead, our method is based on person-specific templates and focuses on capturing space-time coherent challenging human motions using multi-modal references.



\myparagraph{Free-form Volumetric Capture.}
% fusion-based method
Free-form volumetric capture approaches with real-time performance have been proposed by combining the volumetric fusion \cite{Curless1996} and the nonrigid tracking~\cite{sumner2007embedded,li2009robust,zollhofer2014real,guo2015robust} using depth sensors. 
%
The high-end solutions~\cite{dou-siggraph2016,motion2fusion,UnstructureLan,TheRelightables} rely on multi-view studios which are difficult to be deployed.
%
The most handy monocular approaches for general non-rigid scenes~\cite{Newcombe2015,innmann2016volume,guo2017real,KillingFusion2017cvpr,slavcheva2018cvpr,slavcheva2020pami,FlyFusion} 
can only capture small, controlled, and slow motions.
%
Researchers further utilize parametric model~\cite{BodyFusion,DoubleFusion,UnstructureLan,robustfusion} or extra body-worn sensors~\cite{HybridFusion} into the fusion pipeline to increase the tracking robustness.
%
However, these fusion approaches rely on depth cameras which are not as cheap and ubiquitous as color cameras.
% data-driven metthods
Recently, the learning-based techniques enable free-form human reconstruction from monocular RGB input with various representations, such as volume~\cite{DeepHuman_2019ICCV}, silhouette~\cite{SiCloPe_CVPR2019} or implicit representation~\cite{PIFU_2019ICCV,PIFuHD,MonoPort,Chibane_2020CVPR,Implicit_ECCV2020}.
%
However, such data-driven approaches do not recover temporal-coherent reconstruction, especially under the challenging motion setting. 
%
In contrast, our template-based approach can explicitly obtain the per-vertex correspondences over time even for challenging motions.

\myparagraph{Template-based Capture.}
A good compromising settlement between from-form capture and parametric Modal-based Capture is to utilize a specific human template mesh as prior.
%
Early solutions~\cite{Gall2010,StollHGST2011,liu2013markerless,Robertini:2016,Pavlakos17,Simon17,FlyCap} require multi-view capture to produce high quality skeletal and surface motions but synchronizing and calibrating multi-camera systems is still cumbersome. 
%
Recent work only relies on a single-view setup~\cite{MonoPerfCap,LiveCap2019tog,EventCap_CVPR2020} achieve space-time coherent capture and even achieves real-time performance~\cite{LiveCap2019tog}.
%
However, these approaches fail to capture the challenging motions such as yoga or rolling on the floor, which suffer from extreme poses and severe self-occlusion under the monocular setting. 
%
The recent work~\cite{DeepCap_CVPR2020} utilizes weekly supervision on multi-view images directly so as to improve the 3D tracking accuracy during test time.
%
However, their training strategy leads to dedicated per-performer training.
%
Similarly, our approach also employs a person-specific template mesh.
%
Differently, we adopt a specific learning-and-optimization framework for challenging human motion capture.
%
Our learning module is supervised on the motion itself instead of the input images of specific performers for improving the generation performance to various performers and challenging motions. 
%\textcolor{red}{[Ma: How could we achieve the generalization for various performers? Do we explain it in other parts?]}


\begin{figure*}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/fig_3_network}
	\caption{Illustration of our hybrid motion network,  HybridNet, which encodes the global and local temporal motion information with the losses on both the generator and the discriminator. Note that the attention pooling operation is performed by applying element-wise addition (blue branches) on the features of the adjacent body joints. The features after attention pooling are concatenated together with the global feature as input to the fully connected layers.}
	%\textcolor{red}{[Ma: Could we mark the encoder and decoder areas and the discriminator to make the structure clearer? $L_{mc}$ loss equals to $L_{D}$? It is better to unify the representation or give explanation. In addition, give more description in the caption.]}
	\label{fig:fig_3_network}
\end{figure*}

